On the robustness of ChatGPT in teaching Korean Mathematics

ChatGPT, an Artificial Intelligence model, has the potential to revolutionize education. However, its effectiveness in solving non-English questions remains uncertain. This study evaluates ChatGPT's robustness using 586 Korean mathematics questions. ChatGPT achieves 66.72% accuracy, correctly answering 391 out of 586 questions. We also assess its ability to rate mathematics questions based on eleven criteria and perform a topic analysis. Our findings show that ChatGPT's ratings align with educational theory and test-taker perspectives. While ChatGPT performs well in question classification, it struggles with non-English contexts, highlighting areas for improvement. Future research should address linguistic biases and enhance accuracy across diverse languages. Domain-specific optimizations and multilingual training could improve ChatGPT's role in personalized education.

==> _draft_.tex <==

\subsubsection{Challenges and Limitations}
Despite the advancements, several challenges and limitations remain in the ability of VLMs to interpret diagrams effectively:
\begin{itemize}
    \item \textbf{Inaccurate Geometric Perception}: Many MLLMs struggle to accurately perceive basic geometric elements and spatial relationships. This limitation can hinder their ability to solve problems that rely on precise geometric understanding\cite{li2024eagle}.
    \item \textbf{Visual Hallucinations}: MLLMs often generate descriptions that include non-existent objects or inaccurately represent the relationships among existing visual elements, leading to incorrect reasoning\cite{islam2024large}\cite{li2024eagle}\cite{zhang2025mathverse}.
    \item \textbf{Reliance on Textual Cues}: MLLMs often rely heavily on textual cues provided in the problem descriptions rather than interpreting the diagrams, especially if the text is redundant\cite{zhang2025mathverse}\cite{he2024distill}. This reliance undermines their ability to perform true multi-modal reasoning.
    \item \textbf{Limited Scale and Diversity Datasets}: The scale and diversity of current datasets are often insufficient, limiting the potential of VLMs in handling complex multi-modal reasoning tasks\cite{zhang2024mavis}\cite{he2024distill}.

\end{itemize}
